Conjunctive Queries for Logic-Based Information Extraction

This thesis offers two logic-based approaches to conjunctive queries in the context of information extraction. The first and main approach is the introduction of conjunctive query fragments of the logics FC and FC[REG], denoted as FC-CQ and FC[REG]-CQ respectively. FC is a first-order logic based on word equations, where the semantics are defined by limiting the universe to the factors of some finite input word. FC[REG] is FC extended with regular constraints. The second approach is to consider the dynamic complexity of FC.

==> Dynamic/Proofs/proof-beyondsplog.tex <==
\begin{proof}
We prove each of the relations given can be maintained in \dyncq separately.

\paragraph{Maintaining $\scattrelation$:}
Let $u \subwordscatt v$ denote that $u \in \Sigma^*$ is a scattered subword of $v \in \Sigma^*$.
To prove that we can maintain the scattered subword relation in \dyncq, we look at a case distinction, and give a formula to realize each case. 
The update formula is the disjunction of all the given formulas. 
Formally, the relation we maintain is:
\begin{multline*}
\bar R_{\mathsf{scatt}} \df \{ (u_1,u_2,v_1,v_2) \in \worddomain^4 \mid w'[u_1,u_2] \sqsubseteq_{\mathsf{scatt}} w'[v_1,v_2] \text{ and } \\
w'[z] \neq \emptyword \text{ for each } z \in \{ u_1,u_2,v_1,v_2\} \}. 
\end{multline*}

\subparagraph{Part 1 (insertion).}
Consider the insertion of the symbol $\mathtt{a} \in \Sigma$ at position $u \in \worddomain$.
First, we realize the ``base case'' with the following formula. 
\[ \varphi_1 \df \exists z \colon \bigl( R_{\mathtt{a}}(u_1) \land (u_1 \logeq u_2) \land (v_1 \leq z) \land (z \leq v_2) \land R_{\mathtt{a}}(z) \bigr). \]

For $\varphi_1$ to hold, we have that $w'[u_1,u_2] = \mathtt{a}$, and $w'[v_1,v_2] = \bar{s}_0 \cdot \mathtt{a} \cdot \bar{s}_1$ for some $\bar{s}_0, \bar{s}_1 \in \Sigma^*$. 
We can therefore see that this is the correct behaviour for this case.

For the inductive step, we have four cases. 
The cases we explore are as follows:
\begin{enumerate}
\item $u \notin [u_1,u_2]$ and $u \notin [v_1,v_2]$,
\item $u \in [u_1,u_2]$ and $v \notin [v_1,v_2]$,
\item $u \notin [u_1,u_2]$ and $v \in [v_1,v_2]$, and
\item $u \in [u_1,u_2]$ and $v \in [v_1,v_2]$.
\end{enumerate}

Cases two, three, and four are split into further sub-cases. 

\begin{description}
\item[Case 1.] $u \notin [u_1,u_2]$ and $u \notin [v_1,v_2]$:
\end{description}
If $w[u_1,u_2] \subwordscatt w[v_1,v_2]$ and $u$ is outside of the interval $[u_1,u_2]$ and $[v_1,v_2]$, then $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$ and therefore $R'_{\mathsf{scatt}}(u_1,u_2,v_1,v_2)$ should holds. This can be realized by the following:

\[ \varphi_2 \df \scattrelation(u_1,u_2,v_1,v_2) \land (u \notin [u_1,u_2]) \land (u \notin [v_1,v_2]). \]

We use the shorthand $u \notin [u_1,u_2]$ since we have previously realized this behaviour.
If $w[u_1,u_2] \subwordscatt w[v_1,v_2]$ does not hold, and $u \notin [u_1,u_2]$ and $u \notin [v_1,v_2]$, then $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$ also does not hold.

We now move on to the next case.

\begin{description}
\item[Case 2.] $u \in [u_1,u_2]$ and $u \notin [v_1,v_2]$:
\end{description}
We split this case into three subcases.
One case for $u = u_1$, one case for $u_1 < u < u_2$, and one case for $u = u_2$.
Notice that $\varphi_1$ handles the case where $u = u_1 = u_2$ and therefore we can safely assume that $u_1 < u_2$.

\underline{Case 2.1.} $u_1 = u$:


Considering the update $\ins{\mathtt{a}}{u}$, if $w[x_1,u_2] \subwordscatt w[x_2,v_2]$, where $u_1 = u$ such that $u \newnextsym x_1$, and there is some $v$ such that $v_1 \leq v < x_2$ where $w'(u) = w'(v)$, then $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$ (as long as $u \notin [v_1,v_2]$). We realize this case with the following formula:

\begin{multline*}
 \varphi_3 \df  \exists x_1, x_2, v \colon \bigl( \scattrelation(x_1, u_2, x_2,v_2) \land (v_1 \leq v < x_2) \land R_{\mathtt{a}}(v) \land \nextrelation'(u,x_1) \land \\
 (u \notin [v_1,v_2]) \land (u \logeq u_1) \bigr).  
 \end{multline*}


\underline{Case 2.2.} $u_1 < u < u_2$:


If $w[u_1,\bar{x}_1] \subwordscatt w[v_1,x_1]$ and $w[\bar{x}_2,u_2] \subwordscatt w[x_2,v_2]$ for some $\bar x_1, \bar x_2 \in \worddomain$, then it follows that $w[u_1,u_2] \subwordscatt w[v_1,v_2]$ if $\bar{x}_1 \newnextsym u \newnextsym \bar{x}_2$, and $w'[u] \subwordscatt w[x_1+1,x_2-1]$. 
That is, there exists some $v$ where $x_1 < v < x_2$ and $w'[v]=w'[u]$.
This can be thought of as being similar to the case illustrated in~\cref{fig:word} (generalized to scattered subwords, rather than equal factors).
We realize this case with the following formula:

\begin{multline*}
\varphi_4 \df \exists x_1, x_2, \bar{x}_1, \bar{x}_2, y \colon \bigl( (u \notin [v_1,v_2]) \land (u_1 < u < u_2) \land \scattrelation(u_1, \bar{x}_1, v_1, x_1) \land \\ \scattrelation(\bar{x}_2, u_2, x_2, v_2) \land  \nextrelation'(\bar{x}_1, u) \land \nextrelation'(u,\bar{x}_2) \land (x_1 < y < x_2) \land R_{\mathtt{a}}(y) \bigr). 
\end{multline*}

As described before, $\nextrelation'(x,y)$ is shorthand for $\updateformula{\nextrelation}{\ins{\mathtt{a}}{u}}{u;x,y}$.


\underline{Case 2.3.} $u_2 = u$:


This case has analogous reasoning to Case 2.1. We realize this case with the following:
\begin{multline*}
 \varphi_5 \df  \exists x_1, x_2, v \colon \bigl(  \scattrelation(u_1,x_1,v_1,x_2) \land (x_2 < v \leq v_2) \land R_{\mathtt{a}}(v) \land \nextrelation'(x_1,u) \land \\ (u \notin [v_1,v_2]) \land (u \logeq u_2) \bigr). 
 \end{multline*}

This concludes Case 2.

\begin{description}
\item[Case 3.] $u \notin [u_1,u_2]$ and $u \in [v_1, v_2]$:
\end{description}

Similarly to Case 2, this case is split into three further subcases: when $u = v_1$, when $v_1 < u < v_2$, and when $v_2 = u$.
The case where $u = v_1 = v_2$ is dealt with by $\varphi_1$.
Consider $\varphi_1$ for the case where $v_1 = z = v_2 = u$.
Thus, we do not consider the case where $v_1 = v_2 = u$.


\underline{Case 3.1.} $v_1 = u$:

We prove this case with the following formula:
\begin{multline*}
\varphi_6 \df \exists x,y,z \colon \bigl(  \scattrelation(x, u_2, y, v_2) \land \nextrelation'(u_1,x) \land (u \logeq v_1) \land (v_1 \leq z < y) \land \\ \bigvee_{\mathtt{b} \in \Sigma} ( R_{\mathtt{b}}(z) \land R_{\mathtt{b}}(u_1) ) \land (u \notin [u_1,u_2])  \bigr). 
\end{multline*}


\underline{Case 3.2.} $v_1 < u < v_2$:

We realize this case with the following formula:
\begin{multline*}
\varphi_8 \df \exists x_1, x_2, \dots, x_6, y \colon \bigl( \scattrelation(u_1, x_1, v_1, x_4) \land \scattrelation(x_3,u_2,x_5,v_2) \land \\ \nextrelation(x_1,x_2) \land \nextrelation(x_2,x_3) 
\land \bigvee_{\mathtt{b} \in \Sigma} \bigl( R_{\mathtt{b}}(x_2)  \land R_{\mathtt{b}}(y) \bigr) \land \\ (x_4 < y < x_5) \land (x_4 < u < x_5) \land (u \notin [u_1,u_2])\bigr).
\end{multline*}

Since this case is slightly more involved than previous cases, we give more explanation regarding $\varphi_8$.
If $\varphi_8$ holds, then the following hold:
\begin{itemize}
\item $w[u_1, x_1]$ is a scattered subword of $w[v_1,x_4]$,
\item $w[x_3, u_2]$ is a scattered subword of $w[x_5,v_2]$,
\item $w'[x_2]$ is a scattered subword of $w'[x_4+1,x_5-1]$,
\item $x_1 \nextsym x_2 \nextsym x_3$, and
\item $u \notin [u_1,u_2]$.
\end{itemize}

Since $x_1 \nextsym x_2 \nextsym x_3$, it follows that $w[u_1,u_2] = w[u_1,x_1] \cdot w[x_2] \cdot w[x_3,u_2]$. 
Furthermore, $w'[v_1,v_2] = w'[v_1,x_4] \cdot w'[x_4+1,x_5-1] \cdot w'[x_5,v_2]$.
Therefore, $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$.


\underline{Case 3.3.} $v_2 = u$:

This is analogous to Case 3.1.
Consider the following formula:
\begin{multline*}
\varphi_6 \df \exists x,y,z \colon \bigl(  \scattrelation(u_1, x, v_1, y) \land \nextrelation'(x,u_2) \land (u \logeq v_2) \land (y < z \leq v_2) \land \\ \bigvee_{\mathtt{b} \in \Sigma} ( R_{\mathtt{b}}(y) \land R_{\mathtt{b}}(u_2) ) \land (u \notin [u_1,u_2])  \bigr). 
\end{multline*}

\begin{description}
\item[Case 4.] $u \in [u_1,u_2]$ and $u \in [v_1,v_2]$:
\end{description}
This is the most involved case, due to the fact that the intervals $[u_1,u_2]$ and $[v_1,v_2]$ must ``overlap''. 
However, due to the following, we can simplify our case distinction:

First consider following straightforward case:
If $v_1 \leq u_1$ and $u_2 \leq v_2$, then $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$, since $w'[u_1,u_2] \sqsubseteq w'[v_1,v_2]$. This is realized with the following:
\[ \varphi_{11} \df (v_1 \leq u_1) \land (u_2 \leq v_2).\]

Furthermore, if $u_1 < v_1$ and $v_2 < u_2$, then $w'[u_1,u_2]$ cannot be a scattered subword of $w'[v_1,v_2]$, because then $w'[v_1,v_2] \sqsubset w'[u_1,u_2]$.
Since it also must be the case that $u \in [u_1,u_2]$ and $u \in [v_1,v_2]$, this limits us to examine the following sub-cases:
\begin{enumerate}
\item $v_1 < u_1$ and $v_2 < u_2$, and
\item $u_1 < v_1$ and $u_2 < v_2$.
\end{enumerate}

We now give a proof for each of these cases.

\underline{Case 4.1} $v_1 < u_1$ and $v_2 < u_2$:


Notice that if $v_1 < u_1$ and $v_2 < u_2$ where $u_1 < u < u_2$ and $v_1 < u < v_2$, then $\positionSym{w'}{u} - \positionSym{w'}{u_1} < \positionSym{w'}{u} - \positionSym{w'}{v_1}$. This leads to the following:
\begin{align*}
& w[u_1,z_1] \cdot w'[u] \cdot w[z_2, z_3] \cdot w'[y_2] \cdot w[z_4,u_2] \\
\subwordscatt \; & w[v_1,x_1] \cdot w'[y_1] \cdot w[x_2,x_3] \cdot w'[u] \cdot w[x_4,v_2],
\end{align*}

where the following hold:
\begin{itemize}
\item $w'[u_1,u_2] = w[u_1,z_1] \cdot w'[u] \cdot w[z_2, z_3] \cdot w'[y_2] \cdot w[z_4,u_2]$, 
\item $w'[v_1,v_2] = w[v_1,x_1] \cdot w'[y_1] \cdot w[x_2,x_3] \cdot w'[u] \cdot w[x_4,v_2]$,
\item $w[u_1,z_1] \subwordscatt w[v_1,x_1]$,
\item $w[z_2, z_3] \subwordscatt w[x_2,x_3]$,
\item $w[z_4,u_2] \subwordscatt w[x_4,v_2]$,
\item $w'[y_1] = w'[u]$, and
\item $w'[y_2] = w'[u]$.
\end{itemize}

Then, it follows that $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$. This can be realized by the following formula:
 
\begin{multline*}
\varphi_{11} \df \exists z_1,x_1,\dots,z_4,x_4,y_1,y_2 \colon \bigl( \scattrelation(u_1,z_2,v_1,x_1) \land \scattrelation(z_2,z_3,x_2,x_3) \land \\ \scattrelation(z_4,u_2,x_4,v_2) \land
R_{\mathtt{a}}(y_1) \land R_{\mathtt{a}}(y_2) \land \nextrelation'(z_1,u) \land \nextrelation'(u,z_2) \land \\ 
\nextrelation'(z_3,y_2) \land \nextrelation'(y_2,z_4) \land \nextrelation'(x_1,y_1) \\ \land \nextrelation'(y_1,x_2) \land \nextrelation'(x_3,u) \land \nextrelation'(u,x_4) \bigr) 
\end{multline*}

We also have the case where $w[z_2,z_3] = \emptyword$. 
For this case, consider the following:
\begin{center}
	\begin{tabular}{cccccccccc}
		& $w[u_1, z_1]$ & $w'[u]$ & $\emptyword$ & $w'[z_2]$ & $w[z_3,u_2]$,\\
		$\subwordscatt$ & $w[v_1,x_1] $ & $w'[x_2]$ & $w[x_3,x_4] $ & $w'[u]$ & $w[x_5,v_2]$.
	\end{tabular}
\end{center}

Which is realized by $\varphi_{12}$:
\begin{multline*}
\varphi_{12} \df \exists z_1,z_2,z_3,x_1,x_2,x_5 \colon \bigl( \scattrelation(u_1,z_1,v_1,x_1) \land \scattrelation(z_3,u_2,x_5,v_2)  \land  \nextrelation'(z_1,u) \\ \land \nextrelation'(u,z_2) \land \nextrelation'(z_2,z_3)
\land (x_1<x_2<u<x_5) \land R_{\mathtt{a}}(x_2) \land R_{\mathtt{a}}(v_2) \bigr).  
\end{multline*}

Notice that we do not need to introduce the variables $x_3$ and $v_4$ in $\varphi_{12}$ since $x_2 < u$ is sufficient (due to the fact that $w[u+1,z-1] = \emptyword$).

The cases where $u=u_1$ and $u=v_2$ follow analogously. 
Consider the following:
\begin{center}
	\begin{tabular}{cccccccccc}
				 & $w'[u]$ & $\emptyword$ & $w[z_1,z_2]$ & $\emptyword$ & $w[u_2]$\\
$\subwordscatt$ & $w[v_1, y_1] $ & $\cdots$ & $w[x_1,x_2]$ & $\cdots$ & $w'[y_2, u]$,
	\end{tabular}
\end{center}
where $u=u_1$ and $u=v_2$.
Similarly to previous cases, we can realize this with the following formula:
\begin{multline*}
\varphi_{13} \df \exists z_1,z_2,x_1,x_2,y_1,y_2 \colon \bigl(  \scattrelation(z_1,z_2,x_1,x_2) \land (v_1 \leq y_1 < x_1) \land R_{\mathtt{a}}(y_1) \land\\
 (x_2 < y_2 \leq u) \land R_{\mathtt{a}}(y_2) \land \nextrelation'(u,z_1) \land  \\
 \nextrelation'(z_2,u_2) \land (v_1<z_1<z_2<u) \land (u \logeq u_1) \land (u \logeq v_2) \bigr). 
\end{multline*}
For intuition, $\varphi_{13}$ states that $w[z_1,z_2] \subwordscatt w[x_1,x_2]$, and there exists some position $y_1$, where $v_1 \leq y_1 < x_1$ such that $w'[u_1] =w'[y_1]$, and there exists some position $y_2$, where $x_2 < y_2 \leq v_1$ such that $w'[y_2] = w'[v_2]$. Therefore, it follows that $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$. For the case where $u = u_1$ and $v_1 < u < v_2$, consider the following:
\begin{center}
	\begin{tabular}{cccccccccc}
				 & $w'[u]$ 		    & $w[z_1,z_2]$  & $w[z_3]$ & $w[z_4, u_2]$\\
$\subwordscatt$ & $w[v_1, x_1] $ & $w[x_2,x_3]$ & $w'[u]$   & $w'[x_3, v_2]$,
	\end{tabular}
\end{center}



For the case where $u_1 < u < u_2$ and $u = v_2$, consider the following:
\begin{center}
	\begin{tabular}{cccccccccc}
				 & $w[u_1]$ 	  &  $w[z_1,z_2]$ & $w'[u]$    & $w[z_3, u_2]$\\
$\subwordscatt$ & $w'[u, x_1] $ & $w[x_2,x_3]$  & $w[x_4]$ & $w'[x_5, v_2]$,
	\end{tabular}
\end{center}

Since these cases follow analogously, we do not give formulas to realize them.


\underline{Case 4.2} $u_1 < v_1$ and $u_2 < v_2$:


This case is symmetric to Case 4.1. Consider the following:
\begin{align*}
& w[u_1,z_1] \cdot w'[y_1] \cdot w[z_2, z_3] \cdot w'[u] \cdot w[z_4,u_2] \\
\subwordscatt \; & w[v_1,x_1] \cdot w'[u] \cdot w[x_2,x_3] \cdot w'[y_2] \cdot w[x_4,v_2].
\end{align*}
Observing Case 4.1, it is clear that a subformula that handles this case can be written.
While there are other considerations, such as when $w[z_2, z_3] = \emptyword$, these are analogous to Case 4.1, we omit exploring such cases in detail.

The update formula $\updateformula{\scattrelation}{\absins{\mathtt{a}}}{u; u_1,u_2,v_1,v_2}$ is defined by a disjunction over $\varphi_i$, where each $\varphi_i$ realizes a case.
The update formula also ensures that $u_1, u_2, v_1$, and $v_2$ are all symbol elements. 

\subparagraph{Part 2 (reset).}
We now consider the reset operation. 
Assume $u \in \worddomain$ is being reset. 
Firstly, we deal with some special cases:
\begin{itemize}
\item If $u$ is outside of the intervals $[u_1,u_2]$ and $[v_1,v_2]$, then $\scattrelation(u_1,u_2,v_1,v_2)$ if and only if $R'_{\mathsf{scatt}}(u_1,u_2,v_1,v_2)$. 
\item If $u \in \{u_1,u_2,v_1,v_2 \}$ then  $R'_{\mathsf{scatt}}(u_1,u_2,v_1,v_2)$ should not hold, since $u_1,u_2,v_1,v_2$ must be symbol elements.
\item If $u_1 < u < u_2$ and $u \notin [v_1,v_2]$, then $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$ holds.
\item If $v_1 \leq u_1$ and $u_2 \leq v_2$, then $w'[u_1,u_2] \subwordscatt w'[v_1,v_2]$.
\end{itemize}
As we have considered such cases many times, we omit the update formula. 

Therefore, we only need to consider the cases for which $v_1 < u < v_2$.

\begin{description}
\item[Case 1.] $v_1 < u < v_2$ and $u \notin [u_1,u_2]$:
\end{description}

Consider the following:
\begin{center}
	\begin{tabular}{cccccccccc}
		& $w[u_1, z_1]$ & $\emptyword$ & $w[z_2, u_2]$\\
		$\subwordscatt$ & $w[v_1,x_1] $ & $w'[u]$ & $w[x_2, v_2]$,
	\end{tabular}
\end{center}

such that $w[u_1,z_1] \subwordscatt w[v_1,x_1]$ and $w[z_2,u_2] \subwordscatt w[x_2,v_2]$ where $z_1 \nextsym z_2$ and $x_1 \nextsym u \nextsym x_2$. 
This can be realized by the following formula:
\begin{multline*}
\exists z_1, z_2, x_1, x_2 \colon \bigl( \scattrelation(u_1,z_2,v_1,x_1) \land \scattrelation(z_2,u_2,x_2,v_2) \land \nextrelation(z_1,z_2) \land\\
 \nextrelation(x_1,u) \land \nextrelation(u,x_2) \land (u \notin [u_1,u_2]) \bigr). 
\end{multline*}

\begin{description}
\item[Case 2.] $v_1 < u < v_2$ and $u_1 < u < u_2$:
\end{description}
This case has two sub-cases. We only look at one case in detail, as the other case follows analogously.

\underline{Case 2.1.} $v_1 < u_1$ and $v_2 < u_2$:


Consider the following:
\begin{center}
	\begin{tabular}{cccccccccc}
						 & $w[u_1, z_1]$ & $w'[u]$                 & $w[z_2, z_3]$ & $\emptyword$ & $w[z_4,u_2]$ \\
		$\subwordscatt$ & $w[v_1,x_1] $ & $w'[x_1+1,x_2-1]$ & $w[x_2, x_3]$ & $w'[u]$          & $w[x_4,v_2]$.
	\end{tabular}
\end{center}

This can be realized by the following formula:
\begin{multline*}
\exists x_1,z_1,\dots,x_4,v_4 \colon \bigl(  \scattrelation(u_1,z_1,v_1,x_2) \land \scattrelation(z_2,z_3,x_2,x_3) \land \\ \scattrelation(z_4,u_2,x_4,v_2) \land 
\nextrelation(z_1,u)  \land \nextrelation(u,z_2) \land \nextrelation(z_3,z_4) \land \\ (x_1 < x_2) \land \nextrelation(x_3,u) \land \nextrelation(u,x_4) \bigr).
\end{multline*}

There is also the case where the $w[z_2, z_3] = \emptyword$. For this case, consider the following:
\begin{center}
	\begin{tabular}{cccccccccc}
						 & $w[u_1, z_1]$ & $w'[u ]$   & $\emptyword$ & $w[z_2,u_2]$ \\
		$\subwordscatt$ & $w[v_1,x_1] $ & $w[x_1+1,u-1]$  & $w'[u]$          & $w[x_2,v_2]$,
	\end{tabular}
\end{center}

which can be realized by the following formula:
\begin{multline*}
\exists x_1,v_1,x_2,v_2 \colon \bigl( \scattrelation(u_1,z_2,v_1,x_1) \land \scattrelation(z_2,u_2,x_2,v_2) \land \\ (x_1<u<x_2) \land \nextrelation'(z_1, z_2) \bigr). 
\end{multline*}

\underline{Case 2.2.} $u_1 < v_1$ and $u_2 < v_2$:

This case is analogous to Case 2.1, therefore we omit a detailed explanation.

The update formula for the reset operation (akin to the update formula for the insertion operation) is the disjunction of these subformulas. This concludes the proof for maintaining $\scattrelation$.

\paragraph{Maintaining $\numa$:}
To maintain $\numa$, we first maintain the following relations:
\begin{itemize}
\item $\firsta \df \{ i \in \worddomain \mid w[i] = \mathtt{a} \text{ and for all } j < i, w[j] \neq \mathtt{a} \}$,
\item $\lasta \df \{ i \in \worddomain \mid w[i] = \mathtt{a} \text{ and for all } j > i, w[j] \neq \mathtt{a} \}$,
\item $\nexta \df \{ (i,j) \in \worddomain^2 \mid w[i] =w[j] = \mathtt{a} \text{ where } i < j \text{ and for all } k \in \{i+1,i+1,\dots,j-1\}, w[k] \neq \mathtt{a} \}$.
\end{itemize}

Let $\firsta$ be initialized to $\{ \$ \}$.
To maintain $\firsta$ under the $\ins{\mathtt{a}}{u}$ operation, we use the following:
\[ \updateformula{\firsta}{\absins{\mathtt{a}}}{u;x} \df \bigl( \firsta(x) \land (u > x) \bigr) \lor \bigl( (u \logeq x) \land \exists v \colon (\firsta(v) \land (u < v) ) \bigr). \]

To maintain $\firsta$ under the $\ins{\mathtt{b}}{u}$ operation, for all $\mathtt{b} \in \Sigma \setminus \{ \mathtt{a} \}$, we use the following:
\begin{multline*}
\updateformula{\firsta}{\absins{\mathtt{b}}}{u;x} \df  \bigl( \firsta(x) \land ((u<x) \lor (u>x))\bigr) \lor \bigl( \firsta(u) \land \nexta(u,x) \bigr) \lor \\
 \bigl( \firsta(u) \land \lasta(u) \land (x \logeq \$) \bigr). 
 \end{multline*}

Now consider maintaining $\firsta$ under the reset operation.
\begin{multline*}
\updateformula{\firsta}{\absreset}{u;x} \df \bigl( \firsta(x) \land ( (u>x) \lor (u<x) ) \bigr) \lor \bigl( \firsta(u) \land \nexta(u,x) \bigr) \lor \\ \bigl( \firsta(u) \land \lasta(u) \land (x \logeq \$) \bigr). 
\end{multline*}

Maintaining $\lasta$ is analogous to maintaining $\firsta$. 
Let $\lasta$ be initialized to $\{ 1 \}$. 
First, consider the insertion of an $\mathtt{a}$ at position $u \in \worddomain$.
\[ \updateformula{\lasta}{\absins{\mathtt{a}}}{u;x} \df \bigl( \lasta(x) \land (u < x) \bigr) \lor \bigl( (u \logeq x) \land \exists v \colon (\lasta(v) \land (u > v) ) \bigr). \]

To maintain $\lasta$ under the $\ins{\mathtt{b}}{u}$ operation, for all $\mathtt{b} \in \Sigma \setminus \{ \mathtt{a} \}$, we use the following:
\begin{multline*}
\updateformula{\lasta}{\absins{\mathtt{b}}}{u;x} \df  \bigl( \lasta(x) \land ((u > x) \lor (u < x))\bigr) \lor \bigl( \firsta(u) \land \nexta(x,u) \bigr) \lor \\ \bigl( \lasta(u) \land \firsta(u) \land (x \logeq 1) \bigr). 
\end{multline*}

Now consider maintaining $\lasta$ under the reset operation.
\begin{multline*}
\updateformula{\lasta}{\absreset}{u;x} \df \bigl( \lasta(x) \land ((u > x) \lor (u < x))\bigr) \lor \bigl( \firsta(u) \land \nexta(x,u) \bigr) \lor \\ \bigl( \lasta(u) \land \firsta(u) \land (x \logeq 1) \bigr). 
\end{multline*}

We now consider maintaining $\nexta$. We initialize $\nexta$ to $\emptyset$.
To maintain $\nexta$ under the operation $\absins{\mathtt{a}}$, consider the following update formula:
\begin{multline*}
\updateformula{\nexta}{\absins{\mathtt{a}}}{u;x,y} \df \bigl( \nexta(x,y) \land ((u< x) \lor (u < y)) \bigr) \lor \\
\exists v \colon \bigl( \nexta(x,v) \land (x < u < v) \land (u \logeq y) \bigr) \lor \\
\exists v \colon \bigl( \nexta(x,v) \land (x < u < v) \bigr) \lor \bigl( \lasta(x) \land (x<y) \land (u \logeq y) \bigr) \lor \\
\bigl( \firsta(y) \land (x<y) \land (u \logeq x) \bigr).  
\end{multline*} 
Now consider maintaining $\nexta$ under the $\absins{\mathtt{b}}$ operation, where $\mathtt{b} \in \Sigma \setminus \{\mathtt{a} \}$.
\begin{multline*}
\updateformula{\nexta}{\absins{\mathtt{b}}}{u;x,y} \df \bigl(  \nexta(x,y) \land ( ((u<x) \lor (u>y)) \lor ((x<u) \land (u<y) ) ) \bigr) \lor \\ \bigl( \nexta(x,u) \land \nexta(u,y) \bigr). 
\end{multline*}

In regards to maintaining $\nexta$, inserting the symbol $\mathtt{b}$, for some $\mathtt{b} \in \Sigma \setminus \{\mathtt{a} \}$, and performing a reset operation at position $u$ is essentially the same operation. Therefore, in order to deal with the reset operation, we do the following:
\begin{multline*}
\updateformula{\nexta}{\absreset}{u;x,y} \df \bigl(  \nexta(x,y) \land ( ((u<x) \lor (u>y)) \lor ((x<u) \land (u<y) ) ) \bigr) \lor\\ \bigl( \nexta(x,u) \land \nexta(u,y) \bigr). 
\end{multline*}

Notice that $\updateformula{\nexta}{\absins{\mathtt{b}}}{u;x,y} = \updateformula{\nexta}{\absreset}{u;x,y}$.


Now we consider maintaining $\numa$ under the insertion of $\mathtt{a}$ at position $u$. 
Before maintaining $\numa$ under $\absins{\mathtt{a}}$, we consider a restricted version of the relation which we denote with $\barnuma$.
If $(\oneopen,\oneclose,\twoopen,\twoclose) \in \barnuma$, then $w[\oneopen,\oneclose]_{\mathtt{a}} = w[\twoopen,\twoclose]_{\mathtt{a}}$, and $w[i] = \mathtt{a}$ for each $i \in \{ \oneopen, \oneclose, \twoopen, \twoclose \}$.
Since we have the relations $\firsta$, $\lasta$, and $\nexta$, we can utilize the proof of~\cref{lemma:eqsubstr} with minor changes.
Consider $\updateformula{\absins{\mathtt{a}}}{\equalsubstr}{u;\oneopen,\oneclose,\twoopen,\twoclose}$ as defined in~\cref{lemma:eqsubstr}.

To define $\updateformula{\absins{\mathtt{a}}}{\barnuma}{u;\oneopen,\oneclose,\twoopen,\twoclose}$, we replace atoms of $\updateformula{\absins{\mathtt{a}}}{\equalsubstr}{u;\oneopen,\oneclose,\twoopen,\twoclose}$ using the following:
\begin{itemize}
\item Replace each occurrence of $\equalsubstr(\cdot)$ with $\barnuma(\cdot)$,
\item replace each occurrence of $\firstrel(\cdot)$ with $\firsta(\cdot)$,
\item replace each occurrence of $\lastrel(\cdot)$ with $\lasta(\cdot)$, and
\item replace each occurrence of $\nextrelation(\cdot)$ with $\nexta(\cdot)$.
\end{itemize}

To maintain $\barnuma$ under the $\absreset$ operation, we consider the same procedure of replacing atoms as we did for $\updateformula{\absins{\mathtt{a}}}{\barnuma}{u;\oneopen,\oneclose,\twoopen,\twoclose}$.	
Note that the update formula for $\barnuma$ under the $\absins{\mathtt{b}}$, where $\mathtt{b} \in \Sigma \setminus \{ \mathtt{a} \}$ is the same as the update formula for $\absreset$. 

To generalize from maintaining $\barnuma$ to $\numa$, consider the following:
\begin{multline*}
\updateformula{\numa}{\unknownupdate}{u;u_1,u_2,v_1,v_2} \df \exists \bar{x}_o, \bar{x}_c, \bar{y}_o, \bar{y}_c \colon \bigl( \nexta(\bar{x}_o, \oneopen) \land \nexta(\oneclose, \bar{x}_c) \land \nexta(\bar{y}_o, \twoopen) \land \\
\nexta(\twoclose, \bar{y}_c) \land (\bar{x}_o < u_1 \leq \oneopen) \land  (\oneclose < u_2 \leq \bar{x}_c) \land (\bar{y}_o < v_1 \leq \twoopen) \land \\
(\twoclose \leq v_2 < \bar{y}_c) \land \updateformula{\barnuma}{\unknownupdate}{u;u_1,u_2,v_1,v_2} \bigr) 
\end{multline*}

For intuition, we are stating that $(u_1,u_2,v_1,v_2) \in \numa'$ if $(\oneopen,\oneclose,\twoopen,\twoclose) \in \barnuma$, and there does not exist an element that holds the symbol $\mathtt{a}$ between $u_1$ and $\oneopen$, $\oneclose$ and $u_2$, $v_1$ and $\twoopen$, or $\twoclose$ and $v_2$. 

\paragraph{Maintaining $R_{\mathsf{rev}}$:}

We can maintain this with a simple variation of the update formula which maintains $\equalsubstr$. 
Whenever $\equalsubstr(\cdot)$ is used as a subformula, one would need to use $R_{\mathsf{rev}}(\cdot)$ instead. 
The slightly more involved aspect of altering the update formulas would be to reverse the ordering of certain indices. 
This can be done by checking $y \nextsym x$ instead of $x \nextsym y$ where necessary. 

\paragraph{Maintaining $\bar{R}_{\mathsf{perm}}$:} 

We maintain this relation with the following update formula:

\[\updateformula{\bar{R}_{\mathsf{perm}}}{\unknownupdate}{u;u_1,u_2,v_1,v_2} \df \bigwedge\limits_{\mathtt{a} \in \Sigma} \updateformula{\numa}{\unknownupdate}{u;u_1,u_2,v_1,v_2}. \]

Since we maintain the $\numa$ relation, where $(x_1,y_1,x_2,y_2) \in \numa$ if and only if $w[x_1,y_1]_{\mathtt{a}} = w[x_2,y_2]_{\mathtt{a}}$, to maintain $\bar{R}_{\mathsf{perm}}$, we simply consider $\numa$ for all $\mathtt{a} \in \Sigma$. 

\paragraph{Maintaining $\bar{R}_{<}$:}

We maintain this relation with the following update formula:

\begin{multline*}
\updateformula{\bar{R}_{<}}{\unknownupdate}{u;u_1,u_2,v_1,v_2} \df  \exists x_1 \exists x_2 \colon \big( R_{\mathsf{len}}(u_1,u_2,x_1,x_2)  \land\\
(x_1<v_1) \land (v_1\leq v_2) \land (v_2<x_2) \land \bigwedge_{z \in \{u_1,u_2,v_1,v_2\}} ( \bigvee_{\mathtt{a} \in \Sigma} R_{\mathtt{a}}(z) )  \big). 
\end{multline*}

Hence, each of the relations given in this lemma can be maintained in $\dyncq$. The proofs of $\scattrelation$, $\numa$, and $\bar{R}_{\mathsf{rev}}$ follow (with minor changes) from the proof of~\cref{lemma:eqsubstr}.
\end{proof}



==> Dynamic/Proofs/proof-eqlen.tex <==
\begin{proof}
	To maintain the equal length relation, we take the update formulas from \cref{lemma:eqsubstr} and omit any atoms relating to the symbol of an element of the domain $\worddomain$. We also remove the constraint that the first subword must appear before the second. We also use $\bar{R}_{\mathsf{len}}$ in any update formula, rather than $R_{\mathsf{eq}}$. The only exception to omitting all atoms relating to the symbol of an element, is to ensure that $w[u_1] \neq \emptyword$, $w[u_2] \neq \emptyword$, $w[v_1] \neq \emptyword$, and $w[v_2] \neq \emptyword$. Since the equal length relation is not selectable with core spanners, we have shown that \dyncq can maintain relations that are not selectable with core spanners.
\end{proof}
